Just Say No: Analyzing the Stance of Neural Dialogue Generation in Offensive Contexts

Dialogue models trained on human conversations inadvertently learn to generate toxic responses. In addition to producing explicitly offensive utterances, these models can also implicitly insult a group or individual by aligning themselves with an offensive statement. To better understand the dynamics of contextually offensive language, we investigate the stance of dialogue model responses in offensive Reddit conversations. Specifically, we create ToxiChat, a crowd-annotated dataset of 2,000 Reddit threads and model responses labeled with offensive language and stance. Our analysis reveals that 42% of human responses agree with toxic comments, whereas only 13% agree with safe comments. This undesirable behavior is learned by neural dialogue models, such as DialoGPT, which we show are two times more likely to agree with offensive comments. To enable automatic detection of offensive language, we fine-tuned transformer-based classifiers on ToxiChat that achieve 0.71 F1 for offensive labels and 0.53 Macro-F1 for stance labels. Finally, we quantify the effectiveness of controllable text generation (CTG) methods to mitigate the tendency of neural dialogue models to agree with offensive comments. Compared to the baseline, our best CTG model achieves a 19% reduction in agreement with offensive comments and produces 29% fewer offensive replies. Our work highlights the need for further efforts to characterize and analyze inappropriate behavior in dialogue models, in order to help make them safer. Our code and corpus are available at https://github.com/abaheti95/ToxiChat .

==> intro_old.tex <==
\section{Introduction}
\label{sec:intro}
There has been significant progress in building open-domain dialogue agents using large corpora of public conversations \citep{ritter-etal-2011-data,li2016diversity}.
%For example, Facebook's {\em Blender} chatbot is a 9.4 billion parameter neural network that engages in impressive interactions through a combination of pre-training on Reddit, and fine-tuning on smaller, curated datasets that support specific conversational skills \citep{roller-etal-2021-recipes}.
For example, OpenAI's GPT-3 \citep{NEURIPS2020_1457c0d6} is a 175 billion parameter neural network, trained on a 570GB subset CommonCrawl that is capable of engaging in impressive open-domain dialogues with a user, when prompted appropriately.\footnote{\url{https://beta.openai.com/docs/introduction/conversation}}  However, presenting users with content that is generated by a neural network presents new risks, as it is hard to predict when the model might say something offensive or otherwise harmful.

%Neural dialogue may have the potential to support varied, open-domain conversational agents that are much more natural, like talking to a person.

Toxic language is often context dependent \cite{dinan-etal-2019-build}, making it notoriously difficult for language technologies; text that seems innocuous in isolation may in fact be deeply offensive when considered in the broader context of a conversation.  For example, neural chatbots will often agree with offensive statements, which is clearly undesirable (see examples in Figure \ref{fig:example}). 
The solution employed by current systems, such as GPT-3 or Facebook's Blender chatbot \citep{roller-etal-2021-recipes}, is to stop producing output when offensive inputs are detected \citep{xu2020recipes}.  This is problematic, because today's toxic language classifiers are far from perfect, often generating false positive predictions.  Furthermore, there is evidence that these systems have higher false positive rates on text that is written by minority groups, for example African American English \citep{sap2019risk}.  Rather than completely shutting down, for some applications it may be preferable for the dialogue model to simply avoid agreeing with potentially offensive statements.
%We empirically demonstrate that users of the popular social media platform Reddit often agree with offensive statements made by other users, and when trained on this data, neural dialogue models learn to imitate this bad behavior.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{images/offensive_stance_example_figure_new_cropped.pdf}
    \caption{Example of an offensive comment by a Reddit user followed by three Dialogue model's responses. We also show the stance labels for the responses with respect to the preceding offensive comment.}
    \label{fig:example}
\end{figure}

To better understand how stance is expressed in offensive contexts, we recruited crowd-workers on Amazon Mechanical Turk to annotate a corpus of Reddit conversations that include automatically generated responses from DialoGPT \citep{zhang-etal-2020-dialogpt} and GPT-3.  Posts and comments are annotated with regard to whether they can be considered offensive toward a particular person or group \citep{sap-etal-2020-social}.  We also annotate stance toward each of the previous comments in the thread.  This newly annotated corpus is then analyzed to shed light on the behavior of neural dialogue models in offensive contexts.

Using our annotated corpus, in addition to a set of fine-tuned classifiers, we show that 42\% of human responses in offensive contexts exhibit agreement stance, whereas only 13\% agree with safe comments.  Furthermore, we find that neural chatbots learn to mimic this undesirable behavior - DialoGPT, GPT-3 and Blender are significantly more likely to agree with offensive comments.

Finally, we present initial experiments using two methods that aim to control the stance of automatically generated replies.  Our experiments suggest that attribute conditioning and domain adaptive pretraining can  significantly reduce the number of contextually offensive statements. However, this does not completely eliminate the problem, suggesting the need for further research on controllable stance in neural text generation.

Below is the summary of our main contributions:
\begin{enumerate}
    \item We release {\datasetname} dataset of conversations from Reddit along with responses from two dialogue models annotated with targeted-offensive language and stance labels.
    \item We train and analyze conversational offensive language and stance classifiers.
    \item We conduct preliminary experiments on controlled generation to reduce offensive language generated by dialogue models. Specifically, we tune the dialogue model to generate neutral responses to offensive inputs.
\end{enumerate}
